Tiramisu: Layering Consensus Protocols for Scalable and Secure Blockchains

Cryptocurrencies are poised to revolutionize the modern economy by democratizing commerce. These currencies operate on top of blockchain-based distributed ledgers. Existing permissionless blockchain-based protocols offer unparalleled benefits like decentralization, anonymity, and transparency. However, these protocols suffer in performance which hinders their widespread adoption. In particular, high time-to-finality and low transaction rates keep them from replacing centralized payment systems such as the Visa network. Permissioned blockchain protocols offer attractive performance guarantees, but they are not considered suitable for deploying decentralized cryptocurrencies due to their centralized nature. Researchers have developed several multi-layered blockchain protocols that combine both permissioned and permissionless blockchain protocols to achieve high performance along with decentralization. The key idea with existing layered blockchain protocols in literature is to divide blockchain operations into two layers and use different types of blockchain protocols to manage each layer. However, many such works come with the assumptions of honest majority which may not accurately reflect the real world where the participants may be self-interested or rational. These assumptions may render the protocols susceptible to security threats in the real world, as highlighted by the literature focused on exploring game-theoretic attacks on these protocols. We generalize the "layered" approach taken by existing protocols in the literature and present a framework to analyze the system in the BAR Model and provide a generalized game-theoretic analysis of such protocols. Using our analysis, we identify the critical system parameters required for a distributed ledger's secure operation in a more realistic setting.

==> box_dig.tex <==
\begin{tikzpicture}
    \node (acl) [rectangle, rounded corners, minimum width=3cm, minimum height=1cm,text centered] {Layer 1: Selecting Committee};
    \node (csl) [rectangle, rounded corners, minimum width=3cm, minimum height=1cm,text centered, yshift=2cm] {Layer 2: Committee runs consensus protocol};
    \draw [thick,->,>=stealth] (acl) -- node[anchor=west] {} (csl);
\end{tikzpicture}

==> protocol.tex <==
% \sd{@Sanidhay: can you point to where are you talking about the finality of committe in PoW layer, collusion, and cost in the paper}

\section{\ourproto: Protocol \label{sec:ashwachain}}
\label{sec:ourproto}
In this section, we present an example of a Tiramisu-based protocol, namely \ourproto. ASHWAChain~\cite{Arora2020} is an example of as multi-layered blockchain protocol that fits in the Tiramisu framework. \ourproto\ is a committee-based blockchain protocol in which the committee is being updated regularly. The Access Control Layer of \ourproto\ use Proof-of-Work as a method of sybil-resistance and PBFT~\cite{pbft} towards achieving byzantine agreement in the Consensus Layer. As per analysis using the Tiramisu framework, we show that after selecting secure protocol parameters that ensure game-theoretic soundness the protocol can achieve a throughput of more than 700 transactions per second, more than the claim in the original paper by selecting a smaller committee size but greater Proof-of-Work difficulty. We remark that analysis with out framework is also useful in finding optimal parameters for multi-layered blockchain protocols.%\footnote{A preliminary version of \ourproto\ appeared in a non-archival workshop~\cite{Arora2020}}. 
% \st{We first define the underlying network in it.}

\begin{figure}[t]
% \begin{minipage}[c]{0.5\linewidth}
  \centering
        \includegraphics[scale=0.45]{../images/protocol_figure_final.pdf}
        \caption{\ourproto\ overview at height $i$ }
        \label{fig:protocol}
    % \end{minipage}
% \hfill
% \begin{minipage}[c]{0.5\linewidth}
\end{figure}

% \smallskip
% \st{\noindent\textbf{Network Model.}
% We consider a peer-to-peer network consisting of miners who control nodes in the network. These nodes are denoted by their public-private ($pk, sk$) key pair. Miners are connected by a broadcast network over which they can send messages to everyone.}
% \aj{Update this line.}

\subsection{Access Control Layer}
\label{ssec:pbl}



The Access Control Layer of \ourproto\ use Proof-of-Work as a method of sybil-resistance. Here, ACL consists of a blockchain running a PoW protocol, similar to Bitcoin. Each block at height $i$, i.e., $b_i$, is of the form $b_i = \langle h, d, x, p \rangle$. Here $h = H(b_{i-1})$ is the hash of previous block, $d$ is the difficulty of mining, $x$ is the nonce, and $p$ is the identity controlled by a miner that will join the committee to become a \emph{validator}.%(described in Section~\ref{sec:intro}).

Once a miner mines a block $b$ and it reaches finality, ACL provides a \texttt{proposeBlock}$(b)$ operation to interact with the Consensus Layer (CSL)\footnote{CSL will not accept a block if it is not finalized and can be programmed in the in CSL accordingly}. 
This finality condition is left for the implementation according to protocol requirements. For example, when a block in Bitcoin has 6 block confirmations, it is said to be finalized.

Once the finality condition is met, \texttt{proposeBlock}$(b)$ is available to the miner. Specifically, the miner proposes $b$ to CSL. Note that if more than one valid block is proposed at the same time, then only one of them is accepted. Once $b$ is accepted in CSL, a \texttt{commitBlock}$(b)$ event is triggered in ACL for \texttt{proposeBlock}$(b)$. Post this, the identity $p$ in $b$ joins the CSL. All the miners in ACL acknowledge the addition of this block. The updated chain is then considered to mine further blocks, i.e., each miner will mine on this updated chain in case they were not already doing so.



\begin{figure}[!t]
    \centering
    \includegraphics[width=\columnwidth]{../images/protocol_timeline_final.pdf}
    \caption{Illustration of ASHWAChain's timeline}
    \label{fig:timeline}
\end{figure}

% \begin{figure*}[t]
%     \label{fig:tps}
%     \begin{minipage}[c]{0.50\linewidth}
%     \centering
%         \includegraphics[scale=0.42]{../images/tps1.pdf}
%     \end{minipage}%
%     \begin{minipage}[c]{0.45\linewidth}
%     \centering
%         \includegraphics[scale=0.45]{../images/tps2.pdf}
%         % \label{fig:tps2}
%     \end{minipage}%
%     \caption{Transactions Per Seconds v/s Total nodes} %\sd{increase the font weight and size for visibility}
% \end{figure*}

\subsection{Consensus Layer}
%\st{This layer is responsible for fork-resolution and transaction confirmation.} 
The Consensus Layer of \ourproto\ uses PBFT~\cite{pbft} towards achieving byzantine agreement. PBFT works efficiently in asynchronous distributed systems and is optimized for low overhead time. It is a three-phase protocol that guarantees consistency and liveness~\cite{pbft}. Nodes in a PBFT system are sequentially ordered with one node being the leader and others referred to as backup nodes. For PBFT to function correctly, it requires that the number of Byzantine nodes must strictly less than one-third of the total nodes.


CSL is maintained by a committee of nodes. We refer to the nodes present in the committee as \emph{validators}. CSL comprises a shared state which consists of \textsc{PowChain}, $T$, \textsc{ComChain}, \textsc{TxChain}, $O$ and $B$, which are defined later in this subsection and summarised in Table \ref{tab::SS-1}. This shared state is maintained by the committee of validators running SGMP \cite{sgmp} and PBFT agreement protocols, similar to PeerCensus \cite{peercensus}. The shared state can only be modified by three pre-determined operations: \texttt{powBlock}$(b)$, \texttt{txBlock}$(t)$ and \texttt{comBlock}$(c)$ which are defined in Algorithm~\ref{algo:operations}. For easy reference, summary is provided in Table \ref{tab:SS-2}.

CSL proceeds in epochs where each epoch consists of $n_{CSL}$ rounds. In \ourproto, a round is said to be complete after each commit of the \texttt{powBlock}$(b)$ operation (refer Algorithm \ref{algo:operations}). The committee is \textit{updated} after each epoch. The state \textsc{ComChain} stores a blockchain with each block $c$ containing the list of validators. This state is updated after each epoch with \texttt{comBlock}$(c)$, as defined in Algorithm \ref{algo:operations}. The nodes present in the latest block of \textsc{ComChain} are considered as validators for the current epoch. These nodes are the same as those present in the latest $n_{CSL}$ blocks in the \textsc{PowChain} state, which stores the PoW blockchain from ACL, and is updated with \texttt{powBlock}$(b)$ operation (Algorithm \ref{algo:operations}).

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \begin{algorithm}[t]
% \begin{small}
% \DontPrintSemicolon
% \Begin{
%     \eIf{p = Primary}{
%         Creates any operation and broadcasts\;
%     }{
%         Validate operation, sign and broadcast\;
%     }
%     wait($LatencyTime$)\;

%     \eIf{signed by super-majority}{
%         Append $operation$ to $O$\;
%         Commit $operation$ according to its commit rule\;
%     }{
%         Nothing is committed, RESET\;
%     }
% }
% \caption{Agreement for identity $p$ \label{A1}}
% \end{small}
% \end{algorithm}

A primary validator is selected to run the agreement protocol, formally presented in Algorithm~\ref{algo:agreement}. In \textsc{PowChain}, for chain length $l$ and blocks $(b_1, \dots, b_l)$, the identity in block $b_1$ is considered the $primary$ and in case of Byzantine behaviour, next block in the \textsc{PowChain} will used to select the primary validator, using similar procedures as in PBFT. When the miners proceed to the next round after $b$ is committed in \textsc{PowChain}, the next validator in the committee is considered as primary.

The agreement procedure for an identity $p$ in the committee is explained as follows, formally presented in Algorithm~\ref{algo:agreement}. The Primary validator creates the necessary operation and broadcasts it to the committee. The operation is then validated according to its pre-defined rule in Algorithm \ref{algo:operations}. Validators wait to collect all the messages for a certain time according to network latency. Once the operation is signed by a super-majority \footnote{$\frac{2}{3}^{rd}$ of total validators + 1 as we deploy PBFT.} of validators, they append this operation to operation log $O$. Post this, they commit the operation according to its commit rule as defined in Algorithm \ref{algo:operations}.

\textit{Algorithm \ref{algo:operations}} defines all the operations of the CSL. Validation of any operation involves validating all the signatures, transactions, and the block structure. The \texttt{powBlock}$(b)$ operation is broadcasted by the Primary validator after receiving the \texttt{proposeBlock}$(b)$ request from a miner in the ACL. Then, $b$ is appended to the \textsc{PowChain} once this operation is committed. In \texttt{txBlock}$(t)$ operation, $t$ is the block of transactions and each transaction is of the form $tx = \langle from, to, sign, coins, txFee\rangle$, where $from$ and $to$ are the addresses of sender and recipient, $sign$ is the signature of the sender, $coins$ is the number of coins, and $txFee$ is the transaction fee. Once this operation is committed, all the transactions are applied accordingly by updating the state $B$, which stores the Account Balances. Once all the transactions are applied, the state $T$, which stores the list of validators (who signed the transactions for each $tx$) is updated. Note that $v$ is the validator address in Algorithm~\ref{algo:operations}. Post this, Block Reward $BR$, and the total transaction fee is distributed equally among the validators who signed the respective transactions. Finally, the state \textsc{TxChain}, which stores the transaction blockchain, is updated by appending $t$ to it.
In summary, Figure~\ref{fig:protocol} provides the schematic representation of \ourproto.

%\begin{figure}[h]
%
%    \centering
%    \includegraphics[scale = 0.5]{protocol_image.jpeg}
%    \caption{\ourproto\ Diagram}
%    \label{protocol}
%\end{figure}



% \begin{figure}[t]
%     \centering
%         \includegraphics[scale=0.50]{../images/SecurityAnalysis.png}
%     \caption{For a given $\alpha_A$, required $n_{CSL}^{min}$ such that the probability of the system not being in secure state is $1/X$ }
%         \label{fig:spvspop}
%     % \end{minipage}%
% \end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \iffalse
% \begin{figure}[t]
% \centering
%     \begin{subfigure}{0.50\columnwidth}
%         \centering
%         \includegraphics[scale=0.4]{../images/protocol_image.jpeg}
%         \caption{\ourproto\ Overview}
%         \label{fig:protocol}
%     \end{subfigure}
%     \begin{subfigure}{0.45\columnwidth}
%         \centering
%         \includegraphics[scale=0.40]{../images/SecurityAnalysis.png}
%         \caption{Security Analysis: $n_{CSL}^{min}$ vs $\beta$ for different probability guarantees}
%         \label{fig:spvspop}
%     \end{subfigure}

% \end{figure}

% Differences of \ourproto\ and PeerCensus.
% \begin{itemize}
%     \item \ourproto\ has committee of fixed size, in PeerCensus all nodes participate in PBFT and are ever-growing.
%     \item \ourproto\ has idea of epochs, committee updated after each epoch.
%     \item \ourproto\ considers 3 types of nodes (BAR model)
%     \item \ourproto\ has integrated account balances, in PeerCensus Discoin is built on top of the system.
%     % \item \ourproto\
% \end{itemize}

% Similarities of \ourproto\ and PeerCensus.
% \begin{itemize}
%     \item Blockchain layer with PoW and same process to enter next layer.
%     \item Agreement layer running same consensus protocols (PBFT + SGMP).
%     % \item 
%     % \item same idea that computational power proportional to number of nodes.
% \end{itemize}

% \fi




==> protocol_analysis.tex <==
\section{\ourproto: Analysis} \label{sec:ashwachain_analysis}


We re-iterate that NIC-Conditions depends on, along with the protocol design, implementation, and live-network data. We thus assume a NIC \ourproto\ session for the following analysis. We now analyze the game-theoretic, security, and scalability aspects of \ourproto.

% \begin{figure*}[!t]
%     \begin{minipage}[c]{0.50\linewidth}
%     \centering
%         \includegraphics[scale=0.42]{../images/tps1.png}
%         \label{fig:tps1}
%     \end{minipage}%
%     \begin{minipage}[c]{0.45\linewidth}
%     \centering
%         \includegraphics[scale=0.45]{../images/tps2.png}
%         \label{fig:tps2}
%     \end{minipage}%
%     \caption{Transactions Per Seconds v/s Total nodes}
% \end{figure*}



\subsection{Game-theoretic Analysis}

Now, we present a game-theoretic analysis of a NIC \ourproto\ session based on our game model (Section~\ref{subsec:ga}).

In a committee, we have $n_{CSL} = n_H + n_R + n_B$. Note that, the cost of validation is considered for transaction block in specific. $\phi$ and $c_{val}$ are the number of transactions in one block and the cost to validate one transaction, respectively. As we use PBFT, we have, $n_f = \frac{n_{CSL} + 2}{3}$.

\noindent \textbf{Ensuring NIC-Conditions.} Here, we discuss some useful insights for a protocol designer to ensure a NIC \ourproto\ session. By using $F_{\mathcal{SS}}$ from our security analysis (Section~\ref{subsec:sa}), one can ensure a Secure State of a protocol session with any desired security guarantee i.e. $n_A < n_f$ satisfies with a probability of $1 - \epsilon$. Hence, one can ensure the Faithful Fault Tolerance Condition. From Claim~\ref{claim::prob}, we know that $\delta > 0$. We also observe that $c_{val}$ is typically very less once amortized, i.e., once we set up our mining equipment the cost of verifying a transaction from the blockchain stored in a disk is negligible. From this, we observe that the Maximum Payload Condition can be satisfied in cautious implementation. Finally, since Total-Reward is a protocol parameter, one can always set the parameter to satisfy Minimum Reward Condition. Therefore, we observe that NIC-Conditions can be satisfied with the careful and intelligent implementation. Following from Theorem~\ref{thm::PSNE}, we get the result: $s^*_i = s^2_i$ is a PSNE for all rational nodes.


% \aj{1. delta non zero - proof here}
% \aj{2. consequences of 1}
% \sa{added, @anurag edit accordingly after adding proof of claim 1 (commented out)}


% \aj{where is the cond 3 justification?}

% \aj{where is the proof?} \sa{in tiramisu we have general proof. this is just an extension. now referenced here above.}




%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Security Analysis}
\label{sec:security-analysis}

We now present a security analysis of a NIC \ourproto\ session based on our security model (Section~\ref{subsec:sa}).

As we deploy PBFT to reach consensus, our analysis relies on the standard assumption of PBFT that the protocol will only work correctly if the number of Byzantine nodes in the committee is less than one-third of the committee size. Precisely, we have $n_{f} = \frac{n_{CSL} + 2}{3}$. Moreover, the probability of an adversary joining the committee will be directly proportional to its computation power as we use Proof-of-Work in $ACL$.
% To capture this formally, we define the following.

\noindent \textbf{Ensuring Secure State.} Now following from the process of selecting safe committee size described in Section~\ref{selecting:n}, we have Figure \ref{fig:spvspop} for security analysis of \ourproto. It shows the graph between $n_{CSL}^{min}$, i.e., the minimum number of nodes needed to ensure a secure state with respect to $\alpha_A$ for different probability guarantees. More concretely, Figure~\ref{fig:spvspop} presents the threshold of the committee size required for a given $\alpha_A$, considering different values of $\epsilon$ ranging from $2 \times 10^{-4}$ to $2 \times 10^{-6}$.


\begin{figure}[t]
% \begin{minipage}{0.5\linewidth}
% \begin{subfigure}[b]{0.49\columnwidth}
    \centering
    \includegraphics[scale=0.36]{../images/security_analysis.pdf}
    \caption{For a given $\alpha_A$, $n_{CSL}^{min}$ for different values of $\epsilon$.}
        \label{fig:spvspop}
% \end{subfigure}
\end{figure}


\subsection{Scalability Analysis}
\label{sec:scalability-analysis}

% \begin{figure}[t]\label{fig:tps}
%     \centering
%         \includegraphics[scale=0.42]{../images/tps1.pdf}
%     \caption{Transactions Per Seconds vs. Committee Size} %\sd{increase the font weight and size for visibility}
% \end{figure}

\ourproto\ runs the PBFT agreement protocol, which has $O(n^2)$ time complexity where $n$ is the number of nodes. Thus, the transaction throughput in our protocol will depend on $n_{CSL}$. Yaqin et al. \cite{yaqin-hybrid} show that PBFT can scale up to 200 TPS for 100 nodes, where each transaction's size is 50 bytes. We remark that \ourproto\ provides strong consistency, i.e., a transaction will be considered irreversible once it gets accepted. This feature is in contrast to other cryptocurrencies running PoW and PoS protocols like Bitcoin, Ethereum, etc., which need multiple block confirmations for block finality. As a result, the PBFT agreement protocol is the computational bottleneck in \ourproto. Note that the aforementioned cryptocurrencies handle around 20 TPS. Committee-based blockchains like BitShares and DFINITY handle 18 and 40 TPS, respectively. IOTA \cite{iota} uses a DAG-based protocol and handles up to 50 TPS.


\noindent \textbf{\ourproto\ Scalability.} We ran simulations of PBFT for our analysis. Note that Faithful Fault Tolerance Condition is satisfied for our simulations based on the standard assumption for PBFT, i.e. $n_f = \frac{n_{CSL} + 2}{3}$.
We obtain our results for scalability analysis by running simulations of PBFT \cite{pbft-implementation} with different values of $n_{CSL}$. We consider an average transaction size of 200 bytes, which is between the range for an average transaction size of Ethereum (140 bytes, without including smart-contract operation transactions) \cite{ethereum} and Bitcoin (370 bytes)~\cite{bitcoin_tx_size}. We consider each transaction block of size 16 MB, which can contain around 65,000 transactions on average. The primary identity will broadcast this block to the network, and the committee will reach a consensus on the hash of this block.

% \sa{Need to claim that Condition III is satisfied in our simulations.}
% \sa{For Condition II to be true. It says that the avg block size (in bytes) must be less than equal to $\kappa_R \delta / c_{val}$. We don't know the value of $\delta$. need $\phi$ to be reasonable (100Kb - 1Mb?) need to discuss this.}
Considering these parameters, Table~\ref{tab:avg-block-time} shows the average block-time for different committee sizes. Note that this average is for 30 test runs in our simulation for each committee size. Following from this table and the mentioned parameters, Figure~\ref{fig:tps} shows the Transactions Per Second (TPS) for different committee sizes. We can observe that for $n_{CSL} = 51$, \ourproto\ can support at-least 700 TPS, which is a significant improvement over existing cryptocurrency protocols.

From our security analysis, if we consider $\alpha_A = 0.15$, the fraction of the computational power controlled by the adversary to be 15\%, then for $n_{CSL} = 51$, the system is in a secure state with a probability greater than $1.66 \times 10^{-4}$ (Figure~\ref{fig:spvspop}). One must note that, in Bitcoin, this probability is around $0.5 \times 10^{-4}$ for 10\% computational power with Adversary. This note shows that \ourproto\ can support at-least 700 TPS in a secure state with reasonable parameters and probability guarantees.



\begin{figure}[t]
% \end{minipage}
% \begin{minipage}{0.45\linewidth}
% \begin{subfigure}[b]{0.49\columnwidth}
    \centering
        \includegraphics[scale=0.45]{../images/tps1.pdf}
    \caption{Transactions Per Seconds vs. Committee Size}\label{fig:tps}
    % \sg{mark 51 committie size point in circle...or some way to highlight it}} %\sd{increase the font weight and size for visibility}
% \end{subfigure}
% \caption{Analysis of \ourproto}
% \end{minipage}
\end{figure}

\begin{table}[t]
    \centering
    % \resizebox{\columnwidth}{!}{
    \begin{tabular}{c|cccccccc}
        \textbf{Committee Size} & 21 & 31 & 41 & 51 & 61 & 71 & 81 & 91\\
        \hline
        \textbf{Average block-time (s)} & 9 & 23 & 54 & 114 & 174 & 278 & 420 & 879\\
    \end{tabular}
    % }
    \smallskip
    \caption{Average Block-time}
    \label{tab:avg-block-time}
\end{table}

% \begin{table}[t]
%     \centering
%     % \resizebox{\columnwidth}{!}{
%     \begin{tabular}{c|cccccccc}
%         \textbf{Committee Size} & 21 & 31 & 41 & 51 & 61 & 71 & 81 & 91\\
%         \hline
%         \textbf{Average block-time (s)} & 9 & 23 & 54 & 114 & 174 & 278 & 420 & 879\\
%     \end{tabular}
%     % }
%     \smallskip
%     \caption{Average Block-time}
%     \label{tab:avg-block-time}
% \end{table}

